Pose2Gaze: Eye-body Coordination during Daily Activities for Gaze Prediction from Full-body Poses

Human eye gaze plays a significant role in many virtual and augmented reality (VR/AR) applications, such as gaze-contingent rendering, gaze-based interaction, or eye-based activity recognition. However, prior works on gaze analysis and prediction have only explored eye-head coordination and were limited to human-object interactions. We first report a comprehensive analysis of eye-body coordination in various human-object and human-human interaction activities based on four public datasets collected in real-world (MoGaze), VR (ADT), as well as AR (GIMO and EgoBody) environments. We show that in human-object interactions, e.g. pick and place, eye gaze exhibits strong correlations with full-body motion while in human-human interactions, e.g. chat and teach, a person's gaze direction is correlated with the body orientation towards the interaction partner. Informed by these analyses we then present Pose2Gaze, a novel eye-body coordination model that uses a convolutional neural network and a spatio-temporal graph convolutional neural network to extract features from head direction and full-body poses, respectively, and then uses a convolutional neural network to predict eye gaze. We compare our method with state-of-the-art methods that predict eye gaze only from head movements and show that Pose2Gaze outperforms these baselines with an average improvement of 24.0% on MoGaze, 10.1% on ADT, 21.3% on GIMO, and 28.6% on EgoBody in mean angular error, respectively. We also show that our method significantly outperforms prior methods in the sample downstream task of eye-based activity recognition. These results underline the significant information content available in eye-body coordination during daily activities and open up a new direction for gaze prediction.

==> sections/deprecated.tex <==
\subsection{Eye Movements with respect to the Head}\label{sec:gaze_distribution}

To first understand the general coordination of eye and head movements, we analysed the eye gaze distribution in the head coordinate system. Inspired by prior work~\cite{hu2022ehtask, kothari2020gaze}, we used the head position as the origin and eye movements are analysed in this coordinate system. To this end, we first converted eye gaze positions into visual angles in the horizontal and vertical directions and then calculated their distributions across the whole visual field for both datasets separately. The distributions were smoothed using a Gaussian filter with a sigma of one degree of visual angle~\cite{hu2021fixationnet, hu2022ehtask}.
\autoref{fig:gaze_distribution} (a) and (c) illustrate the distributions of eye gaze positions in the MoGaze and GIMO datasets, respectively. As can be seen in the figure, in both datasets most gaze positions fall into the central region of the visual field.
%We further calculated the centres of the eye gaze distributions and got $(0.4^\circ, 13.2^\circ)$ and $(0.2^\circ, 10.1^\circ)$ for MoGaze and GIMO respectively.
%This centre bias is well-known and reflects that human eye gaze in daily activities exhibits a slight bias towards the upper visual field, which corresponds with prior works~\cite{hu2021fixationnet, hadnett2019effect}.
%To have a more intuitive analysis of eye gaze distributions,
We further used $k$-means clustering with $k=128$ to extract cluster centres from the eye gaze positions.
We can see from the right of \autoref{fig:gaze_distribution} that similar to the gaze positions, the cluster centres of gaze positions are mostly located in the centre of the visual field.
These results confirm earlier findings that gaze behaviour is limited to a small central region of the visual field, i.e., exhibits a strong centre bias, particularly in everyday tasks that involve locomotion [REF].

%The fact that eye movements with respect to the head are limited to a small region (i.e. the central region of the visual field) indicates that eye movements have good agreement with the movements of the head in daily activities.


% figures, [htbp] is used to set the format of our figures.
\begin{figure}[t]
    \centering
    \subfigure[Gaze distribution in MoGaze]{\includegraphics[height=0.42\linewidth]{figures/mogaze_distribution.pdf}} 
    \subfigure[Gaze clusters in MoGaze]{\includegraphics[height=0.42\linewidth]{figures/mogaze_distribution_cluster.pdf}} 
    \subfigure[Gaze distribution in GIMO]{\includegraphics[height=0.42\linewidth]{figures/gimo_distribution.pdf}}
    \subfigure[Gaze clusters in GIMO]{\includegraphics[height=0.42\linewidth]{figures/gimo_distribution_cluster.pdf}}
    \caption{Left: The distributions of eye gaze positions in the eye-in-head coordinate system. Right: The cluster centres extracted from the gaze positions. The eye gaze positions and the cluster centres mostly lie in the central region.
    %and their distributions exhibit a bias towards the upper visual field.
    }\label{fig:gaze_distribution}
\end{figure}


To gain a deeper understanding of the correlations between eye gaze and body orientations, we further analysed the correlations between the amplitudes of the gaze shifts and body movements.
Specifically, we used the angular distance between two adjacent gaze directions as the gaze shift amplitude and the angular distance between two adjacent body directions as the amplitude of body movement.
We calculated the correlation between both amplitudes using Spearman's rank correlation coefficient that measures the monotonic relationship between two variables and outputs a value in the range from $-1$ to $+1$, where $-1$ denotes perfect monotone decreasing relationship, $0$ represents no correlation, and $+1$ indicates perfect monotone increasing relationship.
\autoref{fig:gaze_body_amplitude} \todo{add conclusion here}


% figures, [htbp] is used to set the format of our figures.
\begin{figure}[t]
    \centering
    \subfigure[Gaze-body amplitudes in MoGaze]{\includegraphics[width=0.49\linewidth]{figures/gaze_body_amplitude_mogaze.pdf}} 
    \subfigure[Gaze-body amplitudes in GIMO]{\includegraphics[width=0.49\linewidth]{figures/gaze_body_amplitude_gimo.pdf}}
    \caption{The Spearman's correlations between gaze shift amplitude and the amplitudes of body movements at different time intervals in the (a) MoGaze and (b) GIMO datasets.
    }\label{fig:gaze_body_amplitude}
\end{figure}

To investigate the correlations between eye gaze and the movements of different body parts, we grouped the joints into three different body parts, i.e. Torso, Arm, and Leg.
In MoGaze, Torso consists of the body joints of \textit{base}, \textit{pelvis}, \textit{torso}, \textit{neck}, and \textit{head}, Arm contains \textit{left inner shoulder}, \textit{left shoulder}, \textit{left elbow}, \textit{left wrist}, \textit{right inner shoulder}, \textit{right shoulder}, \textit{right elbow}, and \textit{right wrist}, and Leg includes \textit{left hip}, \textit{left knee}, \textit{left ankle}, \textit{left toe}, \textit{right hip}, \textit{right knee}, \textit{right ankle}, and \textit{right toe}.
In GIMO, Torso contains the body joints of \textit{pelvis}, \textit{spine1}, \textit{spine2}, \textit{spine3}, \textit{neck}, \textit{head}, and \textit{jaw}, Arm includes \textit{left collar}, \textit{left shoulder}, \textit{left elbow}, \textit{left wrist}, \textit{right collar}, \textit{right shoulder}, \textit{right elbow}, and \textit{right wrist}, and Leg consists of \textit{left hip}, \textit{left knee}, \textit{left ankle}, \textit{left foot}, \textit{right hip}, \textit{right knee}, \textit{right ankle}, and \textit{right foot}.

We further calculated the mean cosine similarities between eye gaze and the body joints within each body part
%to represent the correlation between eye gaze and the body part
and obtained $0.46$ for Torso, $0.45$ for Arm, and $0.42$ for Leg in MoGaze and $0.35$ for Torso, $0.33$ for Arm, and $0.27$ for Leg in GIMO.
This suggests that eye gaze is more strongly correlated with with upper body movements (torso and arm) than leg movements.
%and, as such, that eye movements are more strongly coordinated with the movements of the upper human body.

The correlation between gaze and a body part was computed using the mean of the cosine similarities between eye gaze and the body joints within the body part.

% Our work
%To evaluate the potential of using human body movements to generate eye gaze,
To this end we first report comprehensive analyses on the correlation between eye movements and the movements of different body parts including head, torso, arms, and legs on two publicly available datasets: MoGaze~\cite{kratzer2020mogaze} and GIMO~\cite{zheng2022gimo}.
These datasets contain eye and full-body movement data recorded using a marker-based body tracking system and a high-resolution mobile eye tracker during various daily activities.

To the best of our knowledge, we are first to study the coordination of eye movements and the movements of different body parts simultaneously.

Our analyses confirm that eye gaze direction is strongly correlated with head direction but also with the movement of different human body joints, especially those of the arms.

We also find that eye gaze coordinates better with future body movements than current motions.

Based on these findings we present \textit{Pose2Gaze}~-- the first method to generate realistic human gaze behaviour from human full-body poses.
At the core of our method is a novel learning-based eye-body coordination model that combines a graph convolutional neural network (GCN) to extract spatio-temporal body pose features with a convolutional neural network (CNN) to generate human eye gaze.
We compare our method with state-of-the-art gaze prediction methods on the MoGaze and GIMO datasets and show
%for generating eye movements for different daily activities.
%Through extensive experiments we demonstrate 
that our method outperforms these baselines by a large margin on both the MoGaze (X\% improvement) and GIMO datasets (Y\%) in terms of mean angular gaze error\footnote{Source code and trained models will be released upon acceptance.}.
\todo{add three generation tasks}

\vspace{1em}
\noindent
The specific contributions of our work are three-fold:
\begin{itemize}

\item We provide a comprehensive analysis on eye-body coordination in various daily activities and reveal that eye gaze is strongly correlated with body movements, especially with head and arm movements.%, and that eye gaze coordinates better with future body motions.

\item We propose \textit{Pose2Gaze}, a novel eye-body coordination model that combines a spatio-temporal graph convolutional neural network to extract features from human full-body poses and a convolutional neural network to generate human eye gaze.

\item We report extensive experiments on two public datasets for generating eye gaze for different daily activities and demonstrate significant performance improvements over several state-of-the-art methods.
\end{itemize}

In this work we have made an important step towards understanding the correlation between eye and full-body movements in daily activities and generating eye gaze from full-body movements.
%Our analyses and the new method advance research in the fields of virtual reality, human-computer interaction, and human-centred computing in several ways.

%\andreas{the following paragraphs are not wrong but they fall a bit short in making clear what the core/novel contributions/findings are. The first two also already talk about applications - and then you have a dedicated paragraph on applications. This is not ideal IMHO. Think about what is the core take away message(s) for each part (coordination analysis, pose-based gaze generation, applications)}

\paragraph{Eye-body Coordination}
In contrast to prior works that typically focused on the correlation between eye gaze and a particular part of the human body, in this work we comprehensively analysed the coordination of human eye and full-body movements in daily activities and revealed that eye gaze is strongly correlated with body orientations and the directions of body motions (\autoref{sec:analysis}).

Our analyses are significant in that they provide information that are crucial for the development of future applications in the areas of virtual reality, human-computer interaction, and human-centred computing.
Specifically, in addition to generating eye gaze from full-body movements that we have explored in this work, eye-body coordination could also be applied to locomotion prediction in virtual reality~\cite{gandrud2016predicting}, target selection in 3D user interfaces~\cite{sidenmark2019selection}, gaze event classification in the wild~\cite{kothari2020gaze}, as well as task recognition in VR and real world scenarios~\cite{hu2022ehtask}.
%Our analyses also guide future research on the important topic of eye-body coordination in daily activities.


\paragraph{Pose-based Gaze Generation}
Prior methods have typically generated eye gaze from head movements while our method generates eye gaze from full-body poses.
Our method significantly outperforms prior methods on both the MoGaze and GIMO datasets for this task (\autoref{tab:gaze_past}, \autoref{tab:gaze_present}, \autoref{tab:gaze_future}) and the ablation studies validated that each body part contributes to the performance of our method (\autoref{tab:ablation_joints}).
As such, our results revealed that in addition to head movements, other body poses are also important for the generation of realistic eye movements.
With the development of motion capture and motion generation techniques~\cite{bhattacharya2021text2gestures,hasegawa2018evaluation}, it becomes increasingly easy to obtain human full-body poses.
Our approach could be integrated with such motion capture and motion generation techniques to generate realistic eye and full-body movements simultaneously.
As such, our method represents a significant advance in pose-based gaze generation and guides future work on this promising research direction.


\paragraph{Applications of Our Method}
We evaluated our method for three different generation tasks (\autoref{sec:gaze_generation_results}), i.e. generating eye gaze from past, present, and future body poses respectively, which are closely linked to different kinds of applications.
Specifically, generating eye gaze from past body poses is equivalent to the setting of forecasting eye gaze in the future~\cite{hu2020dgaze, hu2021fixationnet} and has great significance for visual attention enhancement~\cite{el2009dynamic}, dynamic event triggering~\cite{hadnett2019effect}, as well as human-human and human-computer interaction \cite{steil2018forecasting,mueller2020anticipating}.
Generating eye gaze from present poses is identical to estimating eye gaze in real time~\cite{hu2019sgaze,koulieris2016gaze} and is the key for gaze-contingent rendering~\cite{hu2019sgaze, hu2020dgaze}, gaze-based interaction~\cite{duchowski2018gaze}, and gaze-guided redirected walking~\cite{sun2018towards}.
Generating eye gaze from future poses can be considered as generating eye gaze in a post-processing mode and is particularly significant for creating and animating virtual humans~\cite{bhattacharya2021text2gestures, ruhland2015review}.
The fact that our method outperforms the state-of-the-art methods by a large margin under all the three different generation settings (\autoref{tab:gaze_past}, \autoref{tab:gaze_present}, \autoref{tab:gaze_future}) demonstrates that our method has great potential for the numerous applications mentioned above.
%\andreas{parts of this you already motivated/said in the part where you introduce the tasks.}

In this work we comprehensively analysed the coordination of human eye and full-body movements in daily activities.
In the analysis of correlation between eye gaze and body orientations, we find that eye gaze has strong correlations with the orientations of different body joints, especially with head directions, and these body orientations are strongly correlated with each other (\autoref{tab:gaze_body_orientation}).
This suggests that head direction itself contains sufficient information for generating eye gaze and there is no need to use all the body orientations.
We also find that there exists little or no time delay between head and eye movements (\autoref{fig:gaze_body_direction}).
This inspires us that in situations even where future head directions are available, it is better to still use head directions at the present time to generate target eye gaze than using future head directions.
In the analysis of correlation between eye gaze and body motions, we find that eye gaze is strongly correlated with full-body motions (\autoref{fig:gaze_joint_correlation}), validating that human full-body poses can be used to generate realistic eye gaze.
We also find that there exists a noticeable time delay between full-body motions and eye gaze (\autoref{fig:gaze_pose_correlation}), suggesting that in situations where future pose information is available, we can use future body motions to improve the performance of eye gaze generation.
